On Finite Blocklength Lossy Source Coding

In this monograph, we review recent advances in second-order asymptotics for lossy source coding, which provides approximations to the finite blocklength performance of optimal codes. The monograph is divided into three parts. In part I, we motivate the monograph, present basic definitions, introduce mathematical tools and illustrate the motivation of non-asymptotic and second-order asymptotics via the example of lossless source coding. In part II, we first present existing results for the rate-distortion problem with proof sketches. Subsequently, we present five generations of the rate-distortion problem to tackle various aspects of practical quantization tasks: noisy source, noisy channel, mismatched code, Gauss-Markov source and fixed-to-variable length compression. By presenting theoretical bounds for these settings, we illustrate the effect of noisy observation of the source, the influence of noisy transmission of the compressed information, the effect of using a fixed coding scheme for an arbitrary source and the roles of source memory and variable rate. In part III, we present four multiterminal generalizations of the rate-distortion problem to consider multiple encoders, decoders or source sequences: the Kaspi problem, the successive refinement problem, the Fu-Yeung problem and the Gray-Wyner problem. By presenting theoretical bounds for these multiterminal problems, we illustrate the role of side information, the optimality of stop and transmit, the effect of simultaneous lossless and lossy compression, and the tradeoff between encoders' rates in compressing correlated sources. Finally, we conclude the monograph, mention related results and discuss future directions.

==> chapters/acks.tex <==

L. Zhou was supported by the National Key Research and Development Program of China under Grant 2020YFB1804800, by the National Natural Science Foundation of China under Grant 62201022, and by a start up fund of Beihang university.

M. Motani was supported in part by the Singapore Ministry of Education under Grant MOE2019-T2-2-171.


The authors would like to thank Lei Yu, Qiaosheng (Eric) Zhang, Zhuangfei Wu and Yiming Wang for proofreading parts of this monograph.

